Socioeconomic determinants of protective behaviors and contact patterns in the post-COVID-19 pandemic era: a cross-sectional study in Italy

Socioeconomic inequalities significantly influence infectious disease outcomes, as seen with COVID-19, but the pathways through which socioeconomic conditions affect transmission dynamics remain unclear. To address this, we conducted a survey representative of the Italian population, stratified by age, gender, geographical area, city size, employment status, and education level. The survey's final aim was to estimate differences in contact and protective behaviors across various population strata, both being key components of transmission dynamics. Our initial insights based on the survey indicate that years after the pandemic began, the perceived impact of COVID-19 on professional, economic, social, and psychological dimensions varied across socioeconomic strata, extending beyond the heterogeneity observed in the epidemiological outcomes of the pandemic. This reinforces the need for approaches that systematically consider socioeconomic determinants. In this context, using generalized models, we identified associations between socioeconomic factors and vaccination status for both COVID-19 and influenza, as well as the influence of socioeconomic conditions on mask-wearing and social distancing. Importantly, we also observed differences in contact behaviors based on employment status while education level did not show a significant association. These findings highlight the complex interplay of socioeconomic and demographic factors in shaping individual responses to public health measures. Understanding these dynamics is essential for developing effective epidemic models and targeted public health strategies, particularly for vulnerable populations.

==> tab_covid_impact.tex <==
\begin{tabular}{|l|l|r|r|}
\toprule
               &    &  Count &  Percentage \\
\midrule

covid\_economic\_imp & abbastanza d’accordo &    274 &       22.83 \\
               & molto d’accordo &    205 &       17.08 \\
               & né d’accordo né in disaccordo &    320 &       26.67 \\
               & per niente d’accordo &    203 &       16.92 \\
               & poco d’accordo &    198 &       16.50 \\ \hline
covid\_social\_imp & abbastanza d’accordo &    358 &       29.83 \\
               & molto d’accordo &    180 &       15.00 \\
               & né d’accordo né in disaccordo &    279 &       23.25 \\
               & per niente d’accordo &    202 &       16.83 \\
               & poco d’accordo &    181 &       15.08 \\ \hline
covid\_psy\_imp & abbastanza d’accordo &    356 &       29.67 \\
               & molto d’accordo &    194 &       16.17 \\
               & né d’accordo né in disaccordo &    255 &       21.25 \\
               & per niente d’accordo &    223 &       18.58 \\
               & poco d’accordo &    172 &       14.33 \\ \hline
covid\_work\_imp & abbastanza d’accordo &    212 &       17.67 \\
               & molto d’accordo &    147 &       12.25 \\
               & né d’accordo né in disaccordo &    250 &       20.83 \\
               & per niente d’accordo &    414 &       34.50 \\
               & poco d’accordo &    177 &       14.75 \\
\bottomrule
\end{tabular}

==> tab_employ.tex <==
\begin{tabular}{llrr}
\toprule
               &    &  Count &  Percentage \\
\midrule
qualification & Diploma scuola media superiore &    819 &       68.25 \\
               & Laurea universitaria breve di 1° livello (3 anni) &    109 &        9.08 \\
               & Laurea universitaria specialistica/laurea vecchio ordinamento &     97 &        8.08 \\
               & Licenza elementare &      1 &        0.08 \\
               & Licenza scuola media inferiore &    128 &       10.67 \\
               & Titolo post-laurea (dottorato/master) &     46 &        3.83 \\
employment & Non so/preferisco non rispondere &      5 &        0.42 \\
               & altro indipendente &     17 &        1.42 \\
               & benestante &      1 &        0.08 \\
               & casalinga/o &    147 &       12.25 \\
               & dirigente, alto funzionario, preside, direttore didattico, docente universitario, magistrato &     16 &        1.33 \\
               & disoccupato e non in cerca di lavoro &     14 &        1.17 \\
               & disoccupato ma in cerca di lavoro &    104 &        8.67 \\
               & impiegato &    336 &       28.00 \\
               & impiegato direttivo/quadro &     54 &        4.50 \\
               & imprenditore &     15 &        1.25 \\
               & in cerca di prima occupazione &      9 &        0.75 \\
               & inabile al lavoro &      7 &        0.58 \\
               & insegnante &     48 &        4.00 \\
               & lavoratore autonomo/artigiano &     40 &        3.33 \\
               & libero professionista &     47 &        3.92 \\
               & operaio o posizione similare &    167 &       13.92 \\
               & pensionato &     65 &        5.42 \\
               & studente &    108 &        9.00 \\
emp\_contract & Lavoro a tempo pieno con contratto a tempo indeterminato &    464 &       38.67 \\
               & Lavoro a tempo pieno con contratto a termine &     49 &        4.08 \\
               & Lavoro a tempo ridotto/part-time con contratto a tempo indeterminato &     79 &        6.58 \\
               & Lavoro a tempo ridotto/part-time con contratto a termine &     25 &        2.08 \\
               & Non so/preferisco non rispondere &      4 &        0.33 \\
employ\_sector & Agricoltura, pesca, silvicoltura &     12 &        1.00 \\
               & Altre attività Professionali (avvocati, notai, architetti, commercialisti...) &     46 &        3.83 \\
               & Attività immobiliari, servizi alle imprese &     22 &        1.83 \\
               & Commercio, artigianato &    137 &       11.42 \\
               & Costruzioni &     67 &        5.58 \\
               & Industria &    119 &        9.92 \\
               & Intermediazione monetaria, finanziaria e assicurazioni &     27 &        2.25 \\
               & Pubblica Amministrazione, difesa, istruzione, sanità e altri servizi pubblici &    158 &       13.17 \\
               & Ristorazione (alberghi, ristoranti e bar, catering...) &     43 &        3.58 \\
               & Servizi domestici e altri servizi privati &     61 &        5.08 \\
               & Trasporto e comunicazioni &     48 &        4.00 \\

\end{tabular}{

==> tab_heatlh.tex <==
\begin{tabular}{llrr}
\toprule
               &    &  Count &  Percentage \\
\midrule
health\_assessment & Bene &    562 &       46.83 \\
               & Male &     53 &        4.42 \\
               & Molto bene &    140 &       11.67 \\
               & Molto male &      9 &        0.75 \\
               & Né bene né male &    418 &       34.83 \\
               & Preferisco non rispondere &     18 &        1.50 \\
health\_chronic & No &    874 &       72.83 \\
               & Preferisco non rispondere &     45 &        3.75 \\
               & Sì &    281 &       23.42 \\

\end{tabular}

==> tab_hh.tex <==
\begin{tabular}{llrr}
\toprule
               &    &  Count &  Percentage \\
\midrule
household & 1 &    183 &       15.25 \\
               & 2 &    342 &       28.50 \\
               & 3 &    401 &       33.42 \\
               & 4 &    222 &       18.50 \\
               & 5 &     45 &        3.75 \\
               & 6 &      6 &        0.50 \\
               & 7 &      1 &        0.08 \\
hh\_child & 1 &    213 &       17.75 \\
               & 2 &    112 &        9.33 \\
               & 3 &      1 &        0.08 \\
               & Nessuno &    691 &       57.58 \\
house\_ownership & Altro (uso gratuito o usufrutto) &     41 &        3.42 \\
               & Di mia proprietà/della mia famiglia &    799 &       66.58 \\
               & Di proprietà dei miei genitori &    149 &       12.42 \\
               & In affitto &    191 &       15.92 \\
               & Preferisco non rispondere &     20 &        1.67 \\
hh\_too\_small & No &    987 &       82.25 \\
               & Sì &    213 &       17.75 \\
hh\_expences\_too\_high & No &    855 &       71.25 \\
               & Sì &    345 &       28.75 \\
hh\_too\_far from\_family & No &    912 &       76.00 \\
               & Sì &    288 &       24.00 \\
hh\_too\_far\_from\_doctor & No &    992 &       82.67 \\
               & Sì &    208 &       17.33 \\
hh\_not\_connected\_pt & No &    716 &       59.67 \\
               & Sì &    484 &       40.33 \\
hh\_poor\_struct\_condition & No &   1013 &       84.42 \\
               & Sì &    187 &       15.58 \\
hh\_income & 12.001\&euro; - 18.000\&euro; &    125 &       10.42 \\
               & 120.001\&euro; - 180.000\&euro; &      3 &        0.25 \\
               & 18.001\&euro;- 24.000\&euro; &    167 &       13.92 \\
               & 1€ - 12.000€ &    127 &       10.58 \\
               & 24.001\&euro; - 30.000\&euro; &    181 &       15.08 \\
               & 30.001\&euro; - 36.000\&euro; &    121 &       10.08 \\
               & 36.001\&euro; - 48.000\&euro; &    103 &        8.58 \\
               & 48.001\&euro; - 60.000\&euro; &     74 &        6.17 \\
               & 60.001\&euro; - 90.000\&euro; &     42 &        3.50 \\
               & 90.001\&euro; - 120.000\&euro; &      9 &        0.75 \\
               & Non so/preferisco non rispondere &    227 &       18.92 \\
               & Oltre 180.000\&euro; &      1 &        0.08 \\
               & minore o uguale a 0€ &     20 &        1.67 \\
\end{tabular}

==> tab_mesure.tex <==
\begin{tabular}{|l|l|r|r|}
\toprule
               &    &  Count &  Percentage \\
\midrule
flu\_vaccine & No &    818 &       68.17 \\
               & Preferisco non rispondere &     16 &        1.33 \\
               & Sì &    366 &       30.50 \\ \hline
covid\_vaccine & 1 &     23 &        1.92 \\
               & 2 &    230 &       19.17 \\
               & 3 &    686 &       57.17 \\
               & No, nessuna &    113 &        9.42 \\
               & Più di 3 &    135 &       11.25 \\
               & Preferisco non rispondere &     13 &        1.08 \\ \hline
mask & Mai &    510 &       42.50 \\
               & Qualche volta &    571 &       47.58 \\
               & Sempre &    119 &        9.92 \\ \hline
social\_distance & Mai &    534 &       44.50 \\
               & Qualche volta &    475 &       39.58 \\
               & Sempre &    191 &       15.92 \\ \hline

\end{tabular}

==> tab_mon_all_wt_no_int_additive.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &   mean &     sd &  hdi\_3\% &  hdi\_97\% \\
\midrule
Intercept                  &  4.172 &  0.202 &   3.779 &    4.530 \\
age\_group[25-34]           & -0.759 &  0.154 &  -1.061 &   -0.491 \\
age\_group[35-44]           & -1.008 &  0.155 &  -1.308 &   -0.728 \\
age\_group[45-54]           & -1.148 &  0.150 &  -1.430 &   -0.881 \\
age\_group[55-65]           & -1.190 &  0.143 &  -1.467 &   -0.937 \\
employment[Unemployed]     & -0.121 &  0.139 &  -0.400 &    0.120 \\
education[Nodegree]        & -0.191 &  0.091 &  -0.356 &   -0.012 \\
gender[Male]               &  0.215 &  0.080 &   0.076 &    0.366 \\
city\_size[10000 - 100000]  &  0.054 &  0.089 &  -0.110 &    0.216 \\
city\_size[100000+]         &  0.083 &  0.110 &  -0.112 &    0.299 \\
country\_area[Northeast]    & -0.366 &  0.123 &  -0.581 &   -0.113 \\
country\_area[Nortwest]     & -0.131 &  0.111 &  -0.337 &    0.075 \\
country\_area[South\_Ilands] & -0.118 &  0.107 &  -0.319 &    0.083 \\
part\_work\_mon[Sì]          &  0.846 &  0.131 &   0.610 &    1.109 \\
cnt\_id\_alpha               &  0.725 &  0.030 &   0.671 &    0.781 \\
\bottomrule
\end{tabular}



==> tab_mon_all_wt_no_int_additive_mass.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &   mean &     sd &  hdi\_3\% &  hdi\_97\% \\
\midrule
Intercept                  &  3.781 &  0.228 &   3.324 &    4.186 \\
age\_group[25-34]           & -0.845 &  0.170 &  -1.165 &   -0.514 \\
age\_group[35-44]           & -0.846 &  0.158 &  -1.143 &   -0.560 \\
age\_group[45-54]           & -1.018 &  0.152 &  -1.294 &   -0.727 \\
age\_group[55-65]           & -1.166 &  0.147 &  -1.425 &   -0.886 \\
employment[Unemployed]     & -0.148 &  0.158 &  -0.443 &    0.149 \\
education[Nodegree]        & -0.223 &  0.096 &  -0.402 &   -0.040 \\
gender[Male]               &  0.214 &  0.079 &   0.066 &    0.361 \\
city\_size[10000 - 100000]  &  0.003 &  0.094 &  -0.165 &    0.185 \\
city\_size[100000+]         &  0.021 &  0.114 &  -0.175 &    0.258 \\
country\_area[Northeast]    & -0.245 &  0.127 &  -0.456 &    0.011 \\
country\_area[Nortwest]     &  0.111 &  0.125 &  -0.130 &    0.340 \\
country\_area[South\_Ilands] & -0.031 &  0.118 &  -0.250 &    0.193 \\
part\_work\_mon[Sì]          &  0.534 &  0.143 &   0.269 &    0.796 \\
cnt\_id\_alpha               &  0.843 &  0.041 &   0.766 &    0.915 \\
\bottomrule
\end{tabular}



==> tab_part_age.tex <==
\begin{tabular}{llr}
\toprule
 & Participant age groups & Number of Participants \\
\midrule
0 & 18-24 & 132 \\
1 & 25-34 & 205 \\
2 & 35-44 & 237 \\
3 & 45-54 & 306 \\
4 & 55-65 & 320 \\
\bottomrule
\end{tabular}


==> tab_sun_all_wt_no_int_additive.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &   mean &     sd &  hdi\_3\% &  hdi\_97\% \\
\midrule
Intercept                  &  4.112 &  0.214 &   3.706 &    4.501 \\
age\_group[25-34]           & -0.269 &  0.166 &  -0.575 &    0.048 \\
age\_group[35-44]           & -0.417 &  0.164 &  -0.718 &   -0.110 \\
age\_group[45-54]           & -0.642 &  0.161 &  -0.941 &   -0.343 \\
age\_group[55-65]           & -1.180 &  0.156 &  -1.491 &   -0.904 \\
employment[Unemployed]     &  0.254 &  0.137 &   0.003 &    0.514 \\
education[Nodegree]        & -0.037 &  0.110 &  -0.233 &    0.173 \\
gender[Male]               &  0.201 &  0.087 &   0.049 &    0.370 \\
city\_size[10000 - 100000]  &  0.071 &  0.103 &  -0.115 &    0.269 \\
city\_size[100000+]         &  0.109 &  0.121 &  -0.111 &    0.343 \\
country\_area[Northeast]    & -0.806 &  0.143 &  -1.079 &   -0.539 \\
country\_area[Nortwest]     & -0.228 &  0.133 &  -0.472 &    0.024 \\
country\_area[South\_Ilands] & -0.551 &  0.128 &  -0.795 &   -0.310 \\
part\_work\_sun[Sì]          &  0.309 &  0.133 &   0.068 &    0.573 \\
cnt\_id\_alpha               &  0.466 &  0.018 &   0.433 &    0.500 \\
\bottomrule
\end{tabular}



==> tab_sun_all_wt_no_int_additive_mass.tex <==
\begin{tabular}{lrrrr}
\toprule
{} &   mean &     sd &  hdi\_3\% &  hdi\_97\% \\
\midrule
Intercept                  &  3.270 &  0.229 &   2.839 &    3.711 \\
age\_group[25-34]           & -0.447 &  0.176 &  -0.764 &   -0.103 \\
age\_group[35-44]           & -0.410 &  0.170 &  -0.756 &   -0.109 \\
age\_group[45-54]           & -0.703 &  0.161 &  -0.985 &   -0.384 \\
age\_group[55-65]           & -0.959 &  0.158 &  -1.248 &   -0.659 \\
employment[Unemployed]     &  0.224 &  0.142 &  -0.064 &    0.481 \\
education[Nodegree]        &  0.019 &  0.114 &  -0.196 &    0.223 \\
gender[Male]               &  0.100 &  0.094 &  -0.066 &    0.280 \\
city\_size[10000 - 100000]  &  0.100 &  0.110 &  -0.100 &    0.303 \\
city\_size[100000+]         &  0.046 &  0.131 &  -0.204 &    0.282 \\
country\_area[Northeast]    & -0.216 &  0.147 &  -0.492 &    0.045 \\
country\_area[Nortwest]     & -0.063 &  0.134 &  -0.302 &    0.190 \\
country\_area[South\_Ilands] & -0.220 &  0.127 &  -0.456 &    0.026 \\
part\_work\_sun[Sì]          &  0.396 &  0.133 &   0.160 &    0.652 \\
cnt\_id\_alpha               &  0.538 &  0.024 &   0.492 &    0.582 \\
\bottomrule
\end{tabular}


